Emission-aware Energy Storage Scheduling for a Greener Grid

Reducing our reliance on carbon-intensive energy sources is vital for reducing the carbon footprint of the electric grid. Although the grid is seeing increasing deployments of clean, renewable sources of energy, a significant portion of the grid demand is still met using traditional carbon-intensive energy sources. In this paper, we study the problem of using energy storage deployed in the grid to reduce the grid's carbon emissions. While energy storage has previously been used for grid optimizations such as peak shaving and smoothing intermittent sources, our insight is to use distributed storage to enable utilities to reduce their reliance on their less efficient and most carbon-intensive power plants and thereby reduce their overall emission footprint. We formulate the problem of emission-aware scheduling of distributed energy storage as an optimization problem, and use a robust optimization approach that is well-suited for handling the uncertainty in load predictions, especially in the presence of intermittent renewables such as solar and wind. We evaluate our approach using a state of the art neural network load forecasting technique and real load traces from a distribution grid with 1,341 homes. Our results show a reduction of >0.5 million kg in annual carbon emissions -- equivalent to a drop of 23.3% in our electric grid emissions.

==> load.tex <==
\mohammad{Add some explanation that we need kind of forecasting as the input to the robust optimization ... Even though there are different existing works, we develop a new forecasting approach using LSTM model ... }

\mohammad{The notations in this section must be changed based on the new set of notations in Section 3.}

%Our algorithm focuses on forecasting day-ahead electric load forecasts at the transformer level. Formally we define our problem as, given past electric load data i.e $(L_1, L_2, L_3,..., L_t)$ where $L_t \in R_{> 0}$  and exogenous data $(x_1, x_2, x_3,... x_t) $ we want to learn a function $f$ that forecast H time intervals in the future. \begin{equation}
%	x_{t+1}, x_{t+2}, .., x_{t + H} = f(L_1, L_2, .. , L_t, x_1, x_2,.., x_t)
%\end{equation}
Load forecasting is a widely studied problem in the smart grid domain. A detailed survey of several approaches can be found in~\cite{kyriakides2007short}. More recently, LSTM based techniques have achieved state-of-the-art accuracy~\cite{kong2017short}. These techniques were used to get future predictions of energy usage at \textit{grid-scale} using historical data. However, in our work, we want to perform load forecasting to predict \textit{transformer-level} energy usage, where along with historical data we use exogenous variables. We know that human energy needs vary with change in temperature. Also, energy usage is dependent on human work schedules~\cite{iyengar2016analyzing}. Thus, we use both temperature and day of the week as exogenous variables. 

Formally, in load forecasting, we need to learn a function $f^{[d]}$ $\forall d \in D$ (i.e. the set if all the transformers in consideration), which uses the load seen during the previous $t$ timestamps, given by $l^{d}_{1}, l^{d}_{2}, ..., l^{d}_{t}$ to forecast the load for the next $k$ timestamp over the 24-hour window, given by $l^{d}_{t+1}, l^{d}_{t+2}, ..., l^{d}_{t+k}$. The function $f^{[d]}$ can additionally leverage temperature estimates for the future $k$ timestamps, given by $\tau_{t+1}, \tau_{t+2}, ..., \tau_{t+k}$ and $\delta$, which is the day of the week. In summary, the regression function uses historical energy data along with exogenous variables and is represented as - 
\begin{align*}
l^{d}_{t+1}, ..., l^{d}_{t+k} = f^{[d]}(l^{d}_{1}, ..., l^{d}_{t}, \tau_{t+1}, ..., \tau_{t+k}, \delta) \quad \forall d \in D
\end{align*}

We evaluated several existing load forecasting approaches (see evaluation section).  Apart from these, we propose two regression techniques. We describe them as follows - 

\textbf{Autoregressive Neural Network~\cite{diaconescu2008use}:}Transformer level load data is noisy in nature. However, we observe that historical load data contains daily and weekly seasonality. It is important to extract the seasonality in the historical data for accurate forecasting. In order to forecast load for time $t + 1$ we use the past $p_1$ timesteps as the input along with loads on past $p_2$ days at time $t + 1$ as well as loads at past $p_3$ weeks at time $t + 1$. Along with the historical load, we include one-hot encoded day of the week exogenous variable as part of feature vector of the neural network. We also use the forecasted temperature at time $t + 1$ as an external regressor. Our forecast at time $t+1$is -
\[l^{d}_{t+1} =\beta \cdot \tau_{t+1} +N(l^d_{t}, l^d_{t-1},.., l^d_{t - p_1}, l^d_{t + 1 - h \cdot p_2}, l^d_{t + 1 - h \cdot p_3}, \delta) \]
To forecast k steps in the future, we use rolling forecasting using past predictions.

\textbf{Seasonal LSTM:} As mentioned earlier, historical load data has multiple seasonalities. In order to capture them, we use different LSTMs for each seasonal component as they can have varying number of lagged values as input. We concatenate the encodings from each LSTM unit to get an encoded embedding. The encoded embedding is then passed through a feed forward layer to get the forecast one step ahead in the future. Similar to Autoregressive Neural Network, we use daily and weekly seasonality along with past $p_1$ timesteps. Below, we describe our LSTM model.

	\[e_1 = LSTM(l^d_{t}, l^d_{t - 1},.., l^d_{t - p_1})\]
	\[e_2 = LSTM(l^d_{t - h}, l^d_{t - 2h},..,l^d_{t - p_2.h})\]
	\[e_3 = LSTM(l^d_{t - h}, l^d_{t - 2h},..,l^d_{t - p_3.h})\]
	\[l^d_{t+1} = NN([e_1, e_2, e_3])\]


%\textbf{Dual-Stage Attention LSTM~\cite{qin2017dual}:} Traditionally, attention based encoder decoder techniques perform well on a variety of sequential learning tasks but they don't use exogenous variables as input. However, Dual-Stage Attention LSTMs can incorporate exogenous variables in their model. 
%In this approach, we have two layers of attention mechanism. The first layer of exogenous variable uses Feed Forward Neural Network to extract the importance of exogenous variables for forecasting load at time $t + 1$. The second layer of attention is used to extract the importance of the encoder states for forecasting. These attention layers are used in conjunction with LSTM Neural Network which act as the encoder and decoder layers.


